Representation of quasi-periodic functions and Hausdorff-Young inequalities for Besicovitch almost periodic functions

For a class of $\mathbb{R}^d$-ations and $\mathbb{Z}^d$-actions on the $n$-dimensional torus $\mathbb{T}^n$, we characterize their unique ergodicity and establish a theorem of Weyl type. This result allows us to establish an isomorphism between the Banach algebra of quasi-periodic functions with spectrum in a given $\mathbb{Z}$-module and the Banach algebra of periodic functions on a torus. This, in return, allows us to give a very simple proof of Hausdorff-Young inequalities for Besicovitch almost periodic functions. The regularity of the parent function of a quasi-periodic function is also studied.

==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{bm}
\usepackage{mathtools}
\usepackage{verbatim}
\usepackage{comment}
\usepackage{multirow} 
\usepackage{xspace, soul, color}
\RequirePackage{hyperref} 
\usepackage{xcolor}
\soulregister{\cite}7 % 注册\cite命令
\soulregister{\citep}7 % 注册\citep命令
\soulregister{\citet}7 % 注册\citet命令
\soulregister{\ref}7 % 注册\ref命令
\setlength{\headheight}{27pt}
\usepackage[numbers,sort&compress]{natbib}
\usepackage{times}
%\usepackage{fontspec}
%\setmainfont{TeX Gyre Termes} %新增的
\usepackage{CJKfntef}
\usepackage{caption}
% \captionsetup{
%   font=small,
%   labelfont=bf,
%   compatibility=false  % 启用兼容模式
% }
% \usepackage[format=plain]{caption}  % 对于 article 类文档
% % 或者
% \usepackage[format=hang]{caption}   % 其他格式
\usepackage{titletoc}
\usepackage{lmodern}
\usepackage{amsmath,bm}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{makecell, rotating}
\usepackage{multirow}
\usepackage{algorithmic}
\usepackage{lipsum}
\usepackage{fix-cm}      % 修复字体大小问题
\usepackage{amssymb}     % 数学符号
\usepackage{graphicx}
\usepackage{epstopdf}
%\usepackage{refcheck}%核对公式参考
\usepackage{algorithmic}
\usepackage{tabularx}
\usepackage{anyfontsize}
\usepackage[caption=false]{subfig}

\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}
% Add a serial/Oxford comma by default.
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbZ}{\mathbb{Z}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\bbT}{\mathbb{T}}
\newcommand{\bx}{\bm{x}}
\newcommand{\by}{\bm{y}}
\newcommand{\bz}{\bm{z}}
\newcommand{\blam}{\bm{\lambda}}
\newcommand{\bp}{\bm{p}}
\newcommand{\bP}{\bm{P}}
\newcommand{\bI}{\bm{I}}
\newcommand{\bh}{\bm{h}}
\newcommand{\bk}{\bm{k}}
\newcommand{\bn}{\bm{n}}
\newcommand{\bu}{\bm{u}}
\newcommand{\bs}{\bm{s}}
\newcommand{\bt}{\bm{t}}
\newcommand{\be}{\bm{e}}
\newcommand{\bell}{\bm{\ell}}
\newcommand{\btau}{\bm{\tau}}
\newcommand{\balpha}{\bm{\alpha}}
\newcommand{\bbeta}{\bm{\beta}}
\newcommand{\bgamma}{\bm{\gamma}}
\newcommand{\hatf}{\widehat{f}}
\newcommand{\jk}[1]{{\color{purple}{#1}}}


% \newtheorem{proof}{Proof}[section]
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{corollary}[theorem]{Corollary}
\newtheorem{defy}[theorem]{Definition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{sample}[theorem]{Example}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{prop}[theorem]{Properties}

\newcommand\tbbint{{-\mkern -16mu\int}}
\newcommand\tbint{{\mathchar '26\mkern -14mu\int}}
\newcommand\dbbint{{-\mkern -19mu\int}}
\newcommand\dbint{{\mathchar '26\mkern -18mu\int}}
\newcommand\bint{
	{\mathchoice{\dbint}{\tbint}{\tbint}{\tbint}}
}
\newcommand\bbint{
	{\mathchoice{\dbbint}{\tbbint}{\tbbint}{\tbbint}}
}
\newcommand*{\avint}{\mathop{\ooalign{$\int$\cr$-$}}}
\newcommand{\ds}{\displaystyle}

\DeclareMathOperator*{\argmin}{\mathrm{argmin}}
\DeclareMathOperator*{\argmax}{\mathrm{argmax}}

\newcommand{\Prox}{\mathrm{Prox}}
\newcommand{\BProx}{\mathrm{BProx}}
\newcommand{\GProx}{\mathrm{GProx}}
\newcommand{\Vect}{\mathrm{Vec}}

% Used for creating new theorem and remark environments
% \newsiamremark{remark}{Remark}
% \newsiamremark{hypothesis}{Hypothesis}
% \crefname{hypothesis}{Hypothesis}{Hypotheses}
% \newsiamthm{claim}{Claim}
% \newsiamremark{fact}{Fact}
% \crefname{fact}{Fact}{Facts}
\usepackage{lineno}  % 如果模板自动加载了lineno
\nolinenumbers       % 关闭行号
% Sets running headers as well as PDF title and authors
\headers{Besicovitch almost periodic functions}{Aihua Fan, Kai Jiang, Pingwen Zhang}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Representation of quasi-periodic functions and Hausdorff-Young inequalities for Besicovitch almost periodic functions}

% Authors: full names plus addresses.
\author{
Aihua Fan\thanks{LAMFA, UMR 7352, University of Picardie, 33 Rue Saint Leu, 80039, Amiens, France. Institute for Math \& AI, Wuhan, Wuhan University, Hubei, 430072, China.}
\and 
Kai Jiang\thanks{School of Mathematics and Computational Science, Hunan Key Laboratory for Computation and Simulation in Science and Engineering, Xiangtan University, Hunan, 411105, China.} 
\and 
Pingwen Zhang
\thanks{School of Mathematical Sciences, Peking University, Beijing, 100871, China. Institute for Math \& AI, Wuhan, Wuhan University, Hubei, 430072, China.}
}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}
\newcommand{\see}[1]{{\color{blue}{#1}}}
\newcommand{\change}[1]{{\color{red}{#1}}}
%% Added on Overleaf: enabling xr
\makeatletter
\newcommand*{\addFileDependency}[1]{% argument=file name and extension
  \typeout{(#1)}% latexmk will find this if $recorder=0 (however, in that case, it will ignore #1 if it is a .aux or .pdf file etc and it exists! if it doesn't exist, it will appear in the list of dependents regardless)
  \@addtofilelist{#1}% if you want it to appear in \listfiles, not really necessary and latexmk doesn't use this
  \IfFileExists{#1}{}{\typeout{No file #1.}}% latexmk will find this message if #1 doesn't exist (yet)
}
\makeatother

\newcommand*{\myexternaldocument}[1]{%
    \externaldocument{#1}%
    \addFileDependency{#1.tex}%
    \addFileDependency{#1.aux}%
}

\definecolor{myred}{rgb}{1,0.8,0.8}
\newcommand{\hlred}[1]{{\sethlcolor{myred}\hl{#1}}}

\definecolor{mycyan}{rgb}{0.5,0.92,1.0}
\newcommand{\hlcy}[1]{{\sethlcolor{mycyan}\hl{#1}}}
\definecolor{mycyan}{rgb}{0.5,0.92,1.0}
\definecolor{mygreen}{rgb}{0.56,0.93,0.56}
\newcommand{\hlgr}[1]{{\sethlcolor{mygreen}\hl{#1}}}

\definecolor{myhl}{rgb}{1.0,0.98,0.56}
\sethlcolor{myhl}


